DinoDroid: Testing Android Apps Using Deep Q-Networks

The large demand of mobile devices creates significant concerns about the quality of mobile applications (apps). Developers need to guarantee the quality of mobile apps before it is released to the market. There have been many approaches using different strategies to test the GUI of mobile apps. However, they still need improvement due to their limited effectiveness. In this paper, we propose DinoDroid, an approach based on deep Q-networks to automate testing of Android apps. DinoDroid learns a behavior model from a set of existing apps and the learned model can be used to explore and generate tests for new apps. DinoDroid is able to capture the fine-grained details of GUI events (e.g., the content of GUI widgets) and use them as features that are fed into deep neural network, which acts as the agent to guide app exploration. DinoDroid automatically adapts the learned model during the exploration without the need of any modeling strategies or pre-defined rules. We conduct experiments on 64 open-source Android apps. The results showed that DinoDroid outperforms existing Android testing tools in terms of code coverage and bug detection.

==> acks.tex <==
\section*{Acknowledgments}
This work was supported in part by NSF grant CCF-1464032.

==> bib/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> bib/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subI{Limitations.}
%
The current implementation in \Name{} does not support item-list,
swipe, or scroll actions. 
%where the elements in the list do not fit entirely within the screen.
%Implementing this function requires \commentty{justify why it is non-trivial
%to implement it and the cost of adding this action}.
%\Name{} also does not support swipe or scroll actions. 
In our experiment, three 
fail-to-be-reproduced 
bug reports (FastAdaptor-113, materialistic-1067,
AIMSICD-816) were due to 
the lack of support on these actions. 
We believe  that
\Name{} can be extended to incorporate these actions with additional engineering effort. 
%Second, our implementation of the dynamic GUI exploration
%relies on Robotium, which may not be the most efficient
%execution engine. We believe that other tools, such as 
%UI Automator~\cite{uiautomator} may be used with appropriate 
%configurations to speed up the efficiency of GUI exploration. 
%
Second, \Name{} cannot handle  concurrency bugs or nondeterministic bugs~\cite{FanSCMLXPS18,async18}. 
In our experiment, three fail-to-be-reproduced  bug reports (Memento-169, ScreenCam-32)
were due to non-determinism and one (ODK-1796)
was due to a concurrency bug. 
For example, 
%the yastore-204 app occasionally
%experienced remote server connection problems (e.g., server hang), causing \Name{} to timeout.
to trigger the crash in ODK-1796, it requires waiting on one screen
for seconds and then clicking the next screen at a very fast speed.
In some cases, heuristics can be added
to handle timing issues, such as allowing specific actions to wait for a certain
time period before exploration. 


Third, \Name{} focuses on reproducing crashes. It does not generate
automated test oracles from
bug reports, so it is not able to automatically reproduce 
non-crash bugs. 
Nevertheless, \Name{} can  still  be useful in reproducing 
non-crashed bugs with certain human interventions. 
For example, during the automated dynamic exploration, 
a developer can observe if a non-crashed
bug (e.g., an error message) is reproduced. 
%
% Among all types of bugs in bug
% reports, app crashes are of particular importance to developers
% because it directly impacts an app's 
% usability~\cite{moran2016automatically}.
%
Fourth,
\Name{}  does not support highly specialized text inputs if the input is
not specified in the bug report. 
%This may limit the exploration capabilities of our tool for certain apps. 
%However, 
Recent approaches in symbolic executions 
may prove useful in overcoming this limitation~\cite{jeon2012symdroid}. 
%Sixth, 
%\Name{} does not handle misspelled words because the
%spell checker provided by SpaCy is not reliable and may
%misguide \Name{} to explore incorrect components. Other robust spell 
%checkers, (e.g., Chrome Spell Checker~\cite{googlespell})
%can be integrated with \Name{} to address this problem. 
Finally, 
%\Name{} requires developers to provide 
%the description involving crash reproducing steps in the bug report.
%analyzes the text involving crash reproducing steps (provided by developers)
%while ignoring the code segments and stack traces in the bug report. 
%Recent work on detecting different types of information 
%from bug reports~\cite{chaparro2017detecting}
%can be leveraged to automate this process.  
\Name{} is targeted at bug reports containing natural language description
of reproducing steps. 
In the absence of reproducing steps, \Name{}  would act as a generic GUI exploration tool (i.e., {\em RD$_D$}
in the experiment). 
%\commentty{\Name{} is limited to bug reports containing reproducing steps.}
%\Name{} requires developers to provide the crash description. 



%\commentty{handle non-step-to-reproduce}

\ignore{Sometimes the key word may be wrong spelled. For example,
  there is a real bug report sentence "StringIndexOutOfBoundsException
  tipying only the "space"". In this sentence, the tipyng should be
  typing.  This wrong spell will block the \Name{} to find the right
  word.  We try some automatically spell correct tool to try to
  correct it.  But they all fail. The spacy consider this word as
  "tipy". At last, we find if we input this sentence into google
  search, the google search will correct it automatically. Currently,
  the google search does not provide the API, the developer can
  correct the spell of bug report by himself or transfer it by google
  search to correct it.  }

\subI{\Name{} Vs. Other Techniques.}
%
%The goal of RQ2 is to assess whether \Name{} is
%cost-effective when compared to similar techniques. 
%Ideally, such an assessment would involve comparisons
%with existing state-of-the-art approaches for reproducing crashes from
%bug reports written by natural language. 
In the experiment, we wished to compare \Name{} with existing state-of-the-art 
approaches for reproducing crashes from bug reports written by natural language. 
There are, however, no existing approaches that have this specific goal. 
A tool called Yakusu~\cite{Fazzini2018} presented 
in a recent paper is probably most related to our approach. 
Yakusu extracts GUI elements from bug reports
and then generates an event sequence to cover these elements
as many as possible.
Unlike \Name{}, Yakusu's final goal  
is translating bug reports into test cases
regardless of whether they can reproduce crashes.
Nevertheless, we 
wanted to run their tool on our subject programs
to see if the scripts generated by Yakusu can reproduce crashes. 

%
Unfortunately, after spending one month 
by one graduate student
and one post-doc researcher with rich Android development and research experience,
we were not able to get the tool working\footnote{We contacted the authors, but have not received active responses.}.  
We  included all 25 bug reports from Yakusu to evaluate
our approach, but only six reports can be used because 
none of the three inspectors was able to
manually reproduce the other 19 bugs.  This could be because
Yakusu's evaluation does not aim to successfully
reproduce bugs, but to translate test cases from bug reports. 

We then reversed engineering Yakusu's 
source code and tried to compare Yakusu and \Name{}
conceptually. 
\Name{} is different from Yakusu in several aspects 
(Section~\ref{sec:related} discusses more).
First, \Name{}'  constructs an event
order tree to guide the exploration toward
triggering crashes.
% \Name{} prioritizes the events in the tree. 
%-- the 
%information extracted by the NLP techniques is only used as
%guidance. \Name{} succeeds only when a crash is found. 
In contrast, Yakusu leverages the conventional 
DFS exploration and the algorithm stops when all GUI components
extracted by the static analysis are explored regardless of
whether the crash is found.  
Therefore, event sequences generated by Yakusu may
not reproduce all relevant crashes (e.g.,  false positives). 

Second, Yakusu uses static analysis 
to identify GUI components that are similar to bug reports from source code. 
%It then dynamically searches for these GUI components until all of them are explored. 
Static analysis is often imprecise because it may skip system-wide
GUI components (file systems, databases).  
Therefore, Yakusu can generate imprecise scripts that fail to reproduce bugs.   
We encountered three such cases in our study (acv-11, opensudoku, and notepad).  
For example, in \href{https://github.com/robotmedia/droid-comic-viewer/issues/11}{acv-11}, 
one step is to choose a system directory  ``/mnt", which cannot be identified
in source code. 
%For example, when a bug report mentions
%a generic action, such as ``back", it would not be identified in the source code
%
%\commentty{need a better example}
In contrast, \Name{} is a purely dynamic approach that 
matches the GUI components directly against the bug reports at runtime. 
Therefore, \Name{} is more transparent (no source code is needed)
and potentially more  precise in generating
reproducing scripts than Yakusu.  

Third, Yakusu does not extract input values for 
editable events. Instead, 
%when an editable event happens, 
it will randomly  send an input.  
It may not reproduce bugs that require specific inputs
mentioned in the bug reports (false negatives).
In contrast, \Name{} defines a 
family of grammar rules that can
systematically identify action, GUI components, and
their associated inputs from bug reports. 
As our study (\hyperref[subsec:obs]{Finding 3}) shows, a non-trivial portion of 
crashes involve specific user inputs. 
Therefore, \Name{} is potentially more effectiveness in handling
such bug reports (5 cases in our study). 

%\commentty{Enumerate other limitations.}

\subI{Threats to Validity.}
%
The primary threat to external validity for this study involves the
representativeness of our apps and bug reports.  However, we do reduce
this threat to some extent by using well-studied apps from
existing research and systematically crawling the bug reports of these
apps to avoid introducing biases.  We cannot claim that our results can be
generalized to all bug reports of all domains though.
%
The primary threat to internal validity involves the confounding
effects of participants. We assumed that the students participating in
the study (for RQ3) were substitutes for developers.  We believe the
assumption is reasonable given that all 12 participants indicated that
they had experience in Android programming. Recent
work~\cite{salman2015students} has also shown that students can
represent professionals in software engineering experiments.
%Likewise, the participants in writing 
%bug reports (RQ4) involve both experienced developers and non-experienced
%developers, and the non-experienced ones indicated that
%they were users of Android apps. 


==> overview.tex <==
\section{Overview}
\label{sec:background}


%\Name{} analyzes the reports to identify
%Android GUI components and their associated information and uses this
%to guide the generation of test scripts that will mimic the behavior
%described in the report.  




\subsection{Observations}
\label{subsec:obs}

As the first step, we spent a month studying a large
number of Android bug reports to understand
their characteristics 
for guiding the design  and implementation of \Name{}. 

We collected Android apps from both Google Code
Archive~\cite{googlecode} and GitHub~\cite{githublink}. 
We crawled the bug reports from the first 50 pages in Google Code,
resulting in 3,208 bug reports. 
We then searched Android apps from GitHub by using the keyworld
``Android", resulting in 21,156 bug reports. 
%
Among all 24,364 bug reports, we used 
keywords, such as ``crash"  and ``exception" to search for reports
involving app crashes. This yielded a total number of 2,570 bug reports. 
The result indicates that \emph{a non-negligible number (10.5\%) of 
bug reports involve app crashes}.  

\Name{} focuses on reproducing app \emph{crashes} from bug reports
\emph{containing textual description of reproducing steps}, so we manually 
analyze the 2,570 crash  bug reports and summarize the 
following findings: 1) 813 bug reports (31.6\%) contain reproducing steps --- 
the maximum is 11 steps, the minimum is 1 step, and the average is
2.29 steps; 2) only 3 out of 813 crashes are related to rotate
action ---
they all occur 1--2 steps right after the rotate; 
3) \commentty{???}  of the 813 crash bug reports (61.6\%) 
require specific user inputs on the editable GUI components
to manifest the crashes --- 40 (8\%) of them 
involve special symbols (e.g., apostrophe,
hyphen); 4) 294 crashes (36.1\%) involve generic
click actions, including \texttt{Back} (87), \texttt{OK} (186), 
\texttt{Done} (13), and \texttt{Cancel} (8). 

%The above findings are used to guide the design and 
%implementation of \Name{}, which will be discussed in 
%later sections. 


\begin{figure}[t]
\centering
\includegraphics[scale=0.2]{figures/report}
\caption{Bug Report for 
\href{https://github.com/milesmcc/LibreNews-Android/issues/22}{ LibreNews issue\#22}}
\label{fig:bugreport}
\vspace*{-20pt}
\end{figure}




\subsection{Design Challenges}

An example bug report is shown in
Fig.~\ref{fig:bugreport}. In this example, the reporter describes the
steps to reproduce the crash in five sentences.  The goal of \Name{}
is to translate this sort of description to the event sequence shown in
Fig.~\ref{fig:steps} for triggering the crash.  
To achieve this goal, our approach must address
four main challenges.  First, what types of information need to be
extracted from a bug report?  Second, how can such information be
extracted from reports written in natural language?  Third, how can
this information, which may vary in specificity and completeness, be
used to reproduce the crash? Fourth, how can this process be done
efficiently in terms of a minimal reproduction sequence and the time
to find this sequence? In the remainder of this section, we provide an
overview of how our approach's design addresses these challenges.
Details and algorithms of our approach are presented in
Section~\ref{sec:approach}.


%\gj{at a high level, I think the ``answers'' to these questions often
  %veer into actually presenting the approach as opposed to giving our
  %insight and clever design decision.  I don't think this is a big
  %deal, but if we needed to, I think we could condense this section
  %further by focusing on that shift.}


\subB{What type of information to extract?}
%
%The first challenge is to identify the types of information that are
%broadly useful for guiding crash reproduction.  
%To identify the types
%of information that would be useful, we first examined a large corpus
%of bug reports. 
From the examination of the 813 bug reports containing
reproducing steps, our insight was that events
that trigger new activities, interact with GUI controls, or provide
values are the key parts of the steps provided by bug reporters.  More
broadly, these actions involve performing ``a type of user action" on
``a particular GUI component" with ``specific values" (if the
component is editable).  Therefore, \emph{action}, \emph{target GUI
  component}, and \emph{input values} are the main elements to be
extracted from bug reports. 

To illustrate, consider the fourth step in
Fig.~\ref{fig:bugreport}. Here, ``change" is the user action,
``Server" is the target GUI component, and ``xxyyzz" is the input
value. 
%For the 5th step, ``click" is the user action and ``refresh" is
%the target GUI component (no input values are applicable).


\subB{How to map bug report into semantic representations of events?}
%
The second design challenge is the extraction of the semantic
representation of the reproducing steps from the bug reports,
defined by a tuple \{action, GUI component, input\}.
%For example, referring again to the fourth step in
%Fig.~\ref{fig:bugreport}, our approach needs to extract the \{action,
%GUI component, input\} tuple as \{``type", ``server address",
%``xxyyzz"\}.
%
A seemingly straightforward solution to this challenge is to use
a simple keyword search to match each sentence in the bug report against
the name (i.e., the displayed text) of the GUI components
 from the app. 
However, keyword search cannot reliably detect input values or the
multitude of syntactical relationships that may exist among user
actions, GUI components, and inputs. 
For example, consider a
sentence ``I click the $help$ button to $show$ the word." If both
$help$ and $show$ happen to be the names of app buttons, a 
keyword search
could identify both $help$ and $show$ to be the target GUI components,
whereas only $help$ has a relationship with the action
\texttt{click}. Moreover, reporters may use new words that do not
match the name of the GUI component 
of the app.  For example, a reporter
may use ``play the film" to describe the ``movie" button.


Our insight is that the extraction process can be formulated 
as a slot
filling problem~\cite{mesnil2015using, slotfilling} in natural language processing
(NLP).  
%\gj{I think we need to define slot filling without using NLP
 % jargon.::} In slot filling, the task is to complete all known
%information about a given query entity~\cite{slotfilling}.  \gj{I
 % didn't understand the following example::} This can be thought of as
%``filling" the Wikipedia infoboxes with concrete text from having read
%a large corpus of text (e.g., from Wikipedia itself). 
With this formulation each element of the event tuple is represented as a semantic
slot and the goal of the approach then becomes to fill the slots with
concrete values from the bug report. Our approach uses a mixture of
NLP techniques and heuristics to carry out the slot filling. 
%Since our
%approach must deal with the complexities of natural language grammar,
%we analyze the text describing bug reproduction of each report using the spaCy dependency
%parser~\cite{spacy2} and identify dependencies and grammatical
%relations among words and phrases in each sentence of the bug
%report. 
Specifically, we use the spaCy dependency parser~\cite{spacy2} to identify
typical grammatical structures that were used in bug reports to
describe the relevant user action, target GUI component, and input
values.  
%We then used this parser to study a corpus of 1600 Android bug
%reports from the Google Code Archive~\cite{googlecode} to identify
%typical grammatical structures that were used in bug reports to
%describe the relevant user action, target GUI component, and input
%values.  
These were codified into 18 typical patterns,
which we summarize and describe in Section~\ref{sec:approach}.
The patterns are used to detect event tuples of a new bug report and fill their 
slots with values. 

To help bridge the lexical gap between the terminology in the
bug report and the actual GUI components, our approach uses word
embeddings computed from a word2vec model~\cite{levy2015improving} to
determine whether two words are semantically related. For example, the
words ``movie" and ``film" have a fairly high similarity.  
%For
%sentences in the bug report where dependency parsing cannot be used
%(e.g., really bad grammar), our approach simply tokenizes the sentence
%and compares the content of the app GUI components with the text
%tokens. Here again, word2vec models are used to bridge any lexical
%gap.





\subB{How to create complete and correct sequences for bug
  reproduction?}
%
A key challenge for our approach is that even good bug reports may be
incomplete or inaccurate.  For example, steps that are considered
obvious may be omitted or forgotten by the reporter.  Therefore, our
approach must be able to fill in these missing steps. Ideally,
information already extracted from the report can be 
used to provide ``hints'' to identify and fill in the missing actions.


%Our insight is that a guided GUI crawl can satisfy this need.  
%To illustrate, consider the situation where our approach has
%successfully navigated to step $n$ of a bug report, but is missing an
%unknown number of actions before it can carry out the action described
%in step $n+1$.  A crawler can explore sequences of GUI actions until
%it finds one that allows it to navigate between these two
%steps. Additionally, the extracted event representation for step $n+1$ can be used
%to help the search recognize when it has arrived at the intended GUI
%state.

Existing GUI crawling tools~\cite{azim2013targeted,hao2014puma,mao2016sapienz,amalfitano2015mobiguitar,yang2013grey}
are not a good fit for this particular need. For example, many existing tools
(e.g., A3E~\cite{azim2013targeted}) use a depth-first search (DFS) to systematically explore the GUI
components of an app. That is, the procedure executes the full
sequence of events until there are no more to click before searching
for the next sequence.  In our experience, this is sub optimal because
if an interaction with an incorrect GUI component is chosen 
(due to a missing step), then the subsequent exploration of sub-paths following
that step will be wasted.  

For our problem domain, a guided DFS with
backtracking is more appropriate.  Using this strategy, our approach
can check at each search level whether GUI components that are more
relevant (i.e., match the bug report) to the target step are appearing and use this information to
identify the next component to explore.  If none of the components are
relevant to the bug report, instead of deepening the exploration,
\Name{} can backtrack to a relevant component in a previous search
level.  This process continues until all relevant components in
previous levels are explored before navigating to the subsequent
levels.


\subB{How to make the reproduction efficient?}
%
Efficiency in the reproduction process is important for developer
acceptance.  An approach that takes too long may not seem worth the
wait to developers, and an approach that generates a needlessly long
sequence of actions may be overwhelming to developers.  These two goals
represent a tradeoff for our approach: identifying the minimal set of
actions necessary to reproduce a crash can require more analysis time.


To achieve a reasonable balance between these two efficiency goals, we
designed a set of optimization strategies and heuristics for our
approach. For the guided crawl, we utilized strategies that included
checking the equivalence of screens and detecting loops to avoid
redundant  backtracking, and prioritizing GUI components to be explored
based on their likelihood of causing bugs.  For minimizing the size of
the sequence of GUI actions, whenever a backtrack was needed, our
approach restarted the search from the home screen of the app and
reset the state of the app.  This avoids a common source of
inefficiency present in other approaches (e.g.,
\cite{azim2013targeted,amalfitano2015mobiguitar,yang2013grey}) that add backtracking steps to
their crawling sequence, which results in an overall much longer
sequence of reproducing actions.  

%We discuss these strategies and
%heuristics in more detail in Section~\ref{subsec:guided}.





==> results.tex <==
\section{Evaluation}
\label{sec:evaluation}





\begin{table}[t]
\centering
\scriptsize
%\addtolength{\tabcolsep}{-4pt}
\setlength{\tabcolsep}{1.5pt}
\caption{\label{tab:objects} RQ1 --- RQ3: Different Techniques and User Study}
\scalebox{0.82}{
%\renewcommand{\arraystretch}{0.9}
\begin{tabular}{|l|c|c||c|c|c||c|c|c||r|r|r||c|} \hline
 \#{\em BR.}
& {\em \# steps} & {\em \# ptn} 
& \multicolumn{3}{c||}{\em Reproduce Success}
& \multicolumn{3}{c||}{\em \# Events in Sequence}
& \multicolumn{3}{c||}{\em Time (Seconds)}
& User
\\
%\hline
%& \multicolumn{1}{c|}{\em Total}
%& \multicolumn{1}{c|}{\em ~Time~~}
%& \multicolumn{1}{c|}{\em Replay }
%& \multicolumn{1}{c|}{\em Bug Description}\\
%\cline{4-6}\cline{8-10}

%& {\em \Name{}~} & {\em Sapienz~} & {\em Monkey~}
%& {\em \Name{}~} & {\em Sapienz~} & {\em Monkey~}
%& {\em \Name{}~} & {\em Sapienz~} & {\em Monkey~}
& &
& {\em RD~} &{\em RD$_N$~} &{\em RD$_D$~}  
& {\em RD~} &{\em RD$_N$~} &{\em RD$_D$~}  
& {\em RD~~} &{\em RD$_N$~} &{\em RD$_D$~} 
& (12) 
\\
\hline
\href{https://github.com/samuelclay/NewsBlur/issues/1053}{newsblur-1053}  & 5 & 7 & $\checkmark$ & $\checkmark$  & $\checkmark$    & 7 & 7   & 7 & 157.6 & 133.5  & 132.3 & 12   \\%newblur
\hline
\href{https://github.com/gsantner/markor/issues/194}{markor-194}& 3 & 1 & $\checkmark$ & N  & N    & 4 & -  & -   & 1180.8 & $>$  & $>$ & 12  \\%markor
\hline
\href{https://github.com/rigid/Birthdroid/issues/13}{birthdroid-13} & 1 & 5  & $\checkmark$ & $\checkmark$  & $\checkmark$    & 5  & 8 & 8  & 106.5 & 483.7 & 1088.5 & 9 \\%birthdroid
\hline
\href{https://bitbucket.org/frigus02/car-report/issues/43/infinity-100-km-and-plot-deathlock}{car-report-43}$\star$ & 4 & 4  & $\checkmark$  & $\checkmark$  & $\checkmark$  & 16 & 16  & 16 & 309.5 & 299.4  & 101  & 8  \\%carrreport
\hline
\href{https://code.google.com/archive/p/opensudoku-android/issues/173}{opensudoku-173} & 8 & 10 & $\checkmark$ & N & N   & 9 & -  & -  & 576.4  & $>$ & $>$  & 10 \\%opensudoku
\hline
\href{https://github.com/robotmedia/droid-comic-viewer/issues/11}{acv-11}$\star$ & 5 & 8  & $\checkmark$ & $\checkmark$ & $\checkmark$   & 8  & 8  & 5 & 500.5  & 489.3 & 2060.1 & 7  \\%ACV
\hline
\href{https://code.google.com/archive/p/anymemo/issues/18}{anymemo-18}  & 1 & 2  & $\checkmark$ & $\checkmark$  & $\checkmark$  & 3 & 3 & 3 & 67.1 & 60.9  & 797.7  & 11  \\%anymemo-default
\hline
\href{https://github.com/helloworld1/AnyMemo/issues/440}{anymemo-440} & 4 & 6& $\checkmark$ & $\checkmark$  & N   & 8  & 3  & -  & 933.9 & 889.4  & -   & 12 \\%anymemo-menu
\hline
\href{https://code.google.com/archive/p/banderlabs/issues/23}{notepad-23}$\star$  & 3 & 3 & $\checkmark$ & $\checkmark$ & $\checkmark$    & 6 & 6 & 6   & 216.2 & 292 & 1731.1  & 11 \\%notepad
\hline
\href{https://github.com/vishnus/Olam/issues/2}{olam-2}$\star$  & 1 & 2 & $\checkmark$ & N  & N  & 2 & -  & -  & 56.7 & $>$ & $>$  & 7 \\%olam1_'
\hline
\href{https://github.com/vishnus/Olam/issues/1}{olam-1}  & 1 & 1 & $\checkmark$ & N & N  & 2 & - & - & 35.2 & $>$ & $>$   & 11 \\%olam_space
\hline
\href{https://github.com/mikepenz/FastAdapter/issues/394}{FastAdapter-394}  & 1 & 0& $\checkmark$  & $\checkmark$ & $\checkmark$   & 1 & 1 & 1   & 47.6 & 27.6 & 445.1 & 9   \\%fastadapter
\hline
\href{https://github.com/milesmcc/LibreNews-Android/issues/22}{LibreNews-22} & 4 & 6  & $\checkmark$ & $\checkmark$ & $\checkmark$   & 6 & 6 & 5  & 113.2 & 138.2 & 728.5  & 12   \\%librenew-refresh
\hline
\href{https://github.com/milesmcc/LibreNews-Android/issues/23}{LibreNews-23} & 6 & 4  & $\checkmark$ & N & N  & 3 & - & -  & 47.7 & $>$ & $>$   & 12 \\%librenew-back
\hline
\href{https://github.com/milesmcc/LibreNews-Android/issues/27}{LibreNews-27} & 4 & 4 & $\checkmark$ & $\checkmark$  & $\checkmark$   & 5  & 5 & 5     & 70.2 & 67.6 & 1074.7 & 11  \\%
\hline
\href{https://github.com/ushahidi/SMSSync/issues/464}{SMSSync-464}   & 2 & 0 & $\checkmark$ & $\checkmark$ & $\checkmark$  & 4  & 4 & 4  & 751   & 703.3 & 5193.8 & 10 \\%sms
\hline
\href{https://github.com/y20k/transistor/issues/63}{transistor-63} & 5 & 8 & $\checkmark$ & $\checkmark$ & $\checkmark$ & 3  & 3 & 3  & 41.1 & 36.6  & 65.1 & 12  \\%transister
\hline
\href{https://github.com/zom/Zom-Android/issues/275}{zom-271}  & 5 & 1 & $\checkmark$ & $\checkmark$ & $\checkmark$  & 5  & 5  & 5    & 125.5 & 115.8 & 507.7 & 11 \\%zom
\hline
\href{https://github.com/kriztan/Pix-Art-Messenger/issues/125}{PixART-125} & 3 & 5  & $\checkmark$ & $\checkmark$ & $\checkmark$ & 5 & 5 & 5    & 576.9    & 649.6 & 1031.6 & 12  \\%pixart-share
\hline
\href{https://github.com/kriztan/Pix-Art-Messenger/issues/127}{PixART-127}$\ast$  & 3 & 5& $\checkmark$ & $\checkmark$ & $\checkmark$  & 5  & 5 & 5  & 137.6 & 147.1 & 991.9 & 12  \\%pixart
\hline
\href{https://github.com/vijai1996/screenrecorder/issues/25}{ScreenCam-25}$\ast$& 3 & 2 & $\checkmark$ & $\checkmark$ & N   & 6  & 6 & -  & 721.7 & 833.3 & $>$  & 11  \\%screencam
\hline
\href{https://code.google.com/archive/p/ventriloid/issues/1}{ventriloid-1} & 3 & 3& $\checkmark$ & N  & N  & 9 & -  & -  & 66.8  & $>$ & $>$ & 11   \\%ventriloid
\hline
\href{https://github.com/nextcloud/news-android/issues/487}{Nextcloud-487}  & 1 & 2& $\checkmark$ & $\checkmark$ &$\checkmark$  & 2 & 2  &2  &  63.3&  72  & 943.8  & 11  \\%Nextcloud
\hline
\href{https://github.com/pires/android-obd-reader/issues/22}{obdreader-22}  & 4 & 0& $\checkmark$ & $\checkmark$ & N  & 8  & 8 & - & 891.7 & 939.7 & $>$  & 12 \\%obdreader
\hline
\href{https://github.com/vestrel00/android-dagger-butterknife-mvp/issues/46}{dagger-46}$\ast$ & 1 & 3 & $\checkmark$ & $\checkmark$ & $\checkmark$    & 1  & 1 & 1  & 31.1 & 26.2 & 20.6 & 12 \\%dagger
\hline
\href{https://github.com/opendatakit/collect/issues/2086}{ODK-2086} & 2 & 3 & $\checkmark$ & $\checkmark$ & $\checkmark$ & 3 & 3 & 3 & 89.6 & 91.2 & 2982  & 12  \\%ODK
\hline
\href{https://github.com/k9mail/k-9/issues/3255}{k9-3255}  & 2 & 5 & $\checkmark$  &  N  & N  & 4  & -  &-  & 177.6 & $>$ & $>$ & 12 \\%k9
\hline
\href{https://github.com/k9mail/k-9/issues/2612}{k9-2612}$\ast$ & 4 & 3 & $\checkmark$ & $\checkmark$ & $\checkmark$  & 2  & 3 & 2 & 103  & 134.6  & 5730.6  & 10 \\ %73
\hline
\href{https://github.com/k9mail/k-9/issues/2019}{k9-2019}$\ast$ & 1 & 0 & $\checkmark$ & $\checkmark$ & $\checkmark$  & 3  & 3 & 3 & 59.5  & 58.1 & 1352.4 & 11  \\ %84
\hline
\href{https://github.com/ankidroid/Anki-Android/issues/4586}{Anki-4586}$\ast$ & 5 & 3 & $\checkmark$ & $\checkmark$ & N  & 7  & 7 & - & 96.6  & 100  & $>$  & 12 \\ 
\hline
\href{https://github.com/HiddenRamblings/TagMo/issues/12}{TagMo-12}$\ast$ & 1 & 2 & $\checkmark$ & $\checkmark$ & $\checkmark$  & 2  & 2  & 2 & 14.8  & 15.7  & 29.5 & 12 \\ 
\hline
\href{https://github.com/openMF/android-client/issues/734}{openMF-734}$\ast$ & 2 & 2 & $\checkmark$ & $\checkmark$ & $\checkmark$  & 2  & 2  & 2 & 81.9  & 83.6& 440.5  & 11 \\ 
\hline
\href{https://github.com/ASU-CodeDevils/FlashCards/issues/13}{FlashCards-13}$\ast$ & 4 & 3 & $\checkmark$ & $\checkmark$  & $\checkmark$  & 3  & 3  & 3 & 63.5  & 93.9 & 93.7 & 12  \\ 
\hline
\href{https://github.com/mikepenz/FastAdapter/issues/113}{FastAdaptor-113}  & 2 & 3 & N  & N & N   & - & - &  - & $>$ &  $>$ & $>$ & ? \\%FastList
\hline
\href{https://github.com/alexstyl/Memento-Calendar/issues/169}{Memento-169}  & 3 & 7 & N  & N & N   & - & - & - & $>$ & $>$ & $>$  & ? \\%Memento-Calendar
\hline
\href{https://github.com/vijai1996/screenrecorder/issues/32}{ScreenCam-32} & 1 & 0 & N  & N & N   & - & - & - & $>$ &  $>$ & $>$ & ? \\%ODK
\hline
\href{https://github.com/opendatakit/collect/issues/1796}{ODK-1796} & 2 & 1 & N  & N & N     & - & -  & - & $>$ & $>$ & $>$ & ? \\%ODK
\hline
\href{https://github.com/CellularPrivacy/Android-IMSI-Catcher-Detector/issues/816}{AIMSICD-816}  & 3 & 2   & N & N & N  & - & - & - & $>$ & $>$ & $>$ & ? \\%AIMSICD
\hline
\href{https://github.com/hidroh/materialistic/issues/1067}{materialistic-76}  & 6 & 7   & N & N & N    & - &  - & - & $>$ & $>$ & $>$ & ? \\
%yastore
\hline
\hline
Summary & - & - & 33 & 26  & 22 & ? & ?  & ? & ?  &  ? & ? & ? \\
\hline
\end{tabular}
}
\begin{flushleft}
RD.= \Name{}.
``$\checkmark$"=Crash reproduced.
``N"=Crash not reproduced.
``-"=Not applicable.
 ``$>$"=exceeded time limit (2 hours).
\end{flushleft}
\normalsize
\vspace*{-5pt}
\end{table}






\ignore{
\begin{figure}[t]
\centering
\includegraphics[scale=0.55]{figures/userstudy}
\caption{Manual reproduction of lower-quality (20\%) bug reports}
\label{fig:userplots}
\vspace*{-5pt}
\end{figure}
}

Table~\ref{tab:objects} summarizes the results of applying \Name{},
\Name{}$_{N}$, and \Name{}$_{D}$ in 
39 out of the 51 bug reports. We did not include the 
remaining 12 crashes because they were failed to be reproduced 
due to the technical limitations of
the two execution engines rather than \Name{}.
For example, Robotium failed to click certain buttons (e.g.,~\cite{241}).  
Columns 3--4 show the number reproducing steps in each bug report
and the  number of grammar patterns applicable to each bug report. 
Columns 5--16 show 
whether the technique successfully reproduced the crash,
the size of the event sequence, and the time each technique took.


\subsubsection{RQ1: Effectiveness and Efficiency of \Name{}}

As Table~\ref{tab:objects} shows, \Name{} reproduced 27 out of 34 crashes; 
a success rate of 79.4\%. The time required to reproduce the crashes ranged from
31 to 1,123 seconds with an average time of 372 seconds and a total
time of 167 minutes.  All four crash bug reports (marked with $\star$)
from the FUSION paper~\cite{moran2015auto}
and five bug reports (marked with $\ast$) from  Yakusu~\cite{Fazzini2018} were successfully
reproduced.  The results indicate that \emph{\Name{} is effective in
reproducing crashes from bug reports}.
The six cases where \Name{} failed will be discussed in Section~\ref{sec:discussion}.
%\commentty{whether ReCDroid is more capable of reproducing
%``simple" bugs as compared to more ``complicated" bugs?}
\commentty{Add false negatives and positives in patterns.}

\ignore{For the six cases where \Name{} failed, we found that the failures
were due to the following reasons. First, \Name{} does not support
scroll or swipe action (FastList-113, materialistic-1067,
AIMSICD-816).  Second, \Name{} cannot deal with non-deterministic
behaviors of the apps (Memento-169, ScreenCam-32, yastore-204).
%Specifically, Memento-169 pops up a different window every time
%\Name{} tries to explore the app's home screen and the content of the
%window misguided the exploration.  ScreenCam-32 requires manually
%uploading a specific video to trigger the crash, which cannot be
%automatically done by \Name{}.  
For example, the yastore-204 app occasionally
experienced remote server connection problems (e.g., server hang) at
certain iterations of the exploration, causing \Name{} to timeout.
Third, \Name{} cannot handle time-sensitive crashes. To trigger the
crash for ODK-1796 (a concurrency bug), requires waiting on one screen
for seconds and then clicking the next screen at a very fast speed.
The limitations are summarized in Section~\ref{sec:discussion}. 
}


\subsubsection{RQ2: The Role of NLP in \Name{}}

When compared \Name{} to \Name{}$_{N}$ 
and \Name{}$_{D}$, 
\Name{}$_{N}$ reproduced 26
of the 33 crashes reproduced by \Name{} and required
?\% more time than \Name{}. 
\Name{}$_{D}$ reproduced even fewer crashes (26) and
it took ?\% more time than \Name{}. 
Overall, these results indicate that \emph{the
use of NLP techniques, including both the grammar patterns
and the dynamic word matching, 
contributed to enhancing the 
effectiveness and efficiency of \Name{}.}

\ignore{
\subsubsection{RQ2: \Name{} Vs. Other Techniques}


When compared \Name{} to the other three baseline techniques, our
results showed that \Name{} successfully reproduced 17, 18, and 17
more crashes than Stoat, Sapienz, and Monkey, respectively.  For the
crashes successfully reproduced by both \Name{} and the baseline
techniques, the size of event sequence generated by \Name{} was 98.9\%
smaller than Stoat, 98.7\% smaller than Sapienz, and 99.9\% smaller
than Monkey.  With regards to efficiency, \Name{} required 88.1\% less
time than Stoat, 82.5\% less than Sapienz, and 80.1\% less than
Monkey.  \emph{These results indicate that \Name{} is more
cost-effective timewise than the state-of-the-art bug detection techniques.}
\commentty{It is because of the use of the hint of NLP that makes
\Name{} better.}

\ignore{
\begin{figure}[t]
\centering
\includegraphics[scale=0.55]{figures/userstudy}
\vspace*{-5pt}
\caption{Cost of Successful Manual Reproduction}
\label{fig:userplots}
%\vspace*{-5pt}
\end{figure}
}
}

\subsubsection{RQ3: Usefulness of \Name{}}

The last column of Table~\ref{tab:objects} shows the number of
participants (out of 12) that successfully reproduced the crashes.
While all crashes were reproduced by the participants, among all 27
crashes reproduced by \Name{}, 15 of them failed to be reproduced by
at least one participant.  For the seven bug reports that \Name{}
failed to reproduce, the success rate of human reproduction is also
low. 
%For example, only one participant was able to reproduce the crash
%in yastore-204.  
One reason for the failures is that developers need to 
manually search for the missing steps, which can be difficult
due to the large number of GUI components. As 
columns 3 and 8 in Table~\ref{tab:objects} indicate, 
in 25 bug reports, the number of described steps is
smaller than the number of events actually needed
for reproducing the crashes. Another reason is because
of the misunderstanding of reproducing steps. 
%
These results suggest that \emph{\Name{} is able to
  reproduce crashes that cannot be reproduced by the expert
  developers.}

%\commentty{Draw boxplots.}
%Since the largest amount of time it took to successfully reproduce
%the crash is 560 seconds, we use 600 seconds to indicate the
%failed-to-reproduce crashes (within 30 minutes) for visualization purposes.%\commentty{need to remove 600}

%

We also compute the 
%The boxplots in Figure~\ref{fig:userplots} report the 
time required for each participant to successfully reproduce all 34 bug reports. The results show that the average time for successful manual
reproduction ranged from 9 seconds to 1,229 seconds, with an average
216 seconds --- 42\% less than the time required for \Name{} on the
successfully reproduced crashes.  Such results are expected as \Name{}
needs to explore a number of events during the reproduction.  However,
\emph{\Name{} is fully automated and can thus reduce the painstaking
effort of developers in reproducing crashes.}  Among all 27 crashed
successfully reproduced by \Name{}, the reproduction time required by
individual participants ranged from 201 to 523 seconds.  In fact, five
out of the 12 participants spent more time (18.5\% on average) than
\Name{}.  
%The results further suggest that \emph{\Name{} can save
 % developers' time.} \gj{I think we should drop this last sentence.
 % It seems like we cherry picked this number to make a point that is
 % undermined by the general results.}



%Rows 2--3 of Table~\ref{tab:user} lists the percentage of bug reports
%successfully reproduced and the total
%time required across individual participates.
The 12 participants were then asked to use \Name{} and indicate
their preferences for the manual vs tool-based approach. We used the
scale \emph{very useful}, \emph{useful}, and \emph{not useful}. Our
results indicated that 7 out of 12 participants found \Name{} very
useful and would always prefer \Name{} to manual reproduction, 4
participants indicated \Name{} is useful, and one participant
indicated that \Name{} is not useful and he would rather manually
reproduce the bug. 
% Interestingly, this participant failed to
%reproduce 5 out of 27 crashes reproduced by \Name{}.  
The 12 participants also suggested that \Name{} is useful in the following
cases: 1) bugs that require many steps to reproduce,
2) bugs that require entering specific inputs to reproduce, 
and 3) bug reports that contain too much information.
%
The above results suggest that \emph{developers generally feel \Name{}
  is useful for reproducing crashes from bug reports and they prefer
  to use \Name{} over manual reproduction.}
%\commentty{why wouldn't a developer reproduce it with the hint of the events? }


\ignore{
\begin{table}[t!]
\vspace{1ex}
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\caption{\label{tab:user} User study for original bug reports}
\scalebox{0.9}{
%\renewcommand{\arraystretch}{0.5}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
{\em Participate} & {\em U1} & {\em U2}
& {\em U3}& {\em U4}& {\em U5}& {\em U6}
& {\em U7}& {\em U8}& {\em U9}& {\em U10}
& {\em U11}& {\em U12}\\
\hline
App. (success) & 25/27 & 27/27& 25/27 & 22/27 & 24/27 &  25/27 & 24/27 & 22/27& 22/27 & 26/27& 26/27 & 25/27
\\
\hline
Time (total) & 7244  & 4758  & 8507 & 11136 & 9024 & 7576 & 9166 & 11672 & 12759 & 5677 & 5352 & 7744
\\
\hline
Useful (score) & 3 & 3 & 3 & 2 & 0 & 3 & 3 & 3 & 3 & 3 & 3 & 3
\\
\hline
\end{tabular}
}
%\normalsize
\vspace*{-5pt}
\end{table}
}


\begin{table}[t]
\centering
\scriptsize
%\addtolength{\tabcolsep}{-4pt}
\setlength{\tabcolsep}{3pt}
\caption{\label{tab:user} RQ4: Different Quality Levels}
%\scalebox{0.88}{
%\renewcommand{\arraystretch}{0.1}
\begin{tabular}{|l|c|r|c|r|c|r|} \hline
 \#{\em BR.}
& \multicolumn{2}{c|}{\em QL-10\% (5)}
& \multicolumn{2}{c|}{\em QL-20\% (5)}
& \multicolumn{2}{c|}{\em QL-50\% (5)}
\\
%\hline
%& \multicolumn{1}{c|}{\em Total}
%& \multicolumn{1}{c|}{\em ~Time~~}
%& \multicolumn{1}{c|}{\em Replay }
%& \multicolumn{1}{c|}{\em Bug Description}\\
%\cline{4-6}\cline{8-10}

%& {\em \Name{}~} & {\em Sapienz~} & {\em Monkey~}
%& {\em \Name{}~} & {\em Sapienz~} & {\em Monkey~}
%& {\em \Name{}~} & {\em Sapienz~} & {\em Monkey~}
& {\em Success} & {\em Time (sec)} & {\em Success} & {\em Time (sec)} & {\em Success} & {\em Time (sec)}
\\
\hline
newsblur-1053   & 5 & 196(102) & 5 & 94(50) & 5 & 136(88) \\%newblur
\hline
markor-194   & 5 & 1601(24) & 4  & 1564(85) & 4 & 1608(30) \\%markor
\hline
birthdroid-13   & 5 & 159(128) & 5 & 383(205) & 5 & 659(185)\\%birthdroid
\hline
car-report-43     & 5 & 280(3) & 5 & 288(6) & 5 & 286(1) \\%carrreport
\hline
opensudoku-173    & 5  & 770(458) & 3 & 2267(1153) & 3 & 2325(1636) \\%opensudoku
\hline
acv-11  & 5 & 1077(1299) & 5 & 1844(1448) & 5 & 1911(1321) \\%ACV
\hline
anymemo-18   & 5  & 90(49) & 5 & 62(9) & 5 & 1527(1009)\\%anymemo-default
\hline
anymemo-440   & 3 & 1570(85) & 3  & 1488(85) & 0 &$>$(-) \\%anymemo-menu
\hline
notepad-23  & 5 & 333(167) & 5 & 683(544) & 5& 920(671) \\%notepad
\hline
olam-2   & 5 & 52(2) & 4 & 50(1) & 3 & 50(1)\\%olam1_'
\hline
olam-1  & 5 & 27(1) & 5 & 27(1) & 3 & 27(1)\\%olam_space
\hline
FastAdapter-394 & 5 & 48(1) & 5 & 455(374) & 5 & 740(8) \\%fastadapter
\hline
LibreNews-22   & 5 & 123(33) & 5 & 176(77) & 5 & 287(239) \\%librenew-refresh
\hline
LibreNews-23  & 2 & 56(12) & 2  & 62(4) & 3 & 108(54) \\%librenew-back
\hline
LibreNews-27   & 5& 93(3)  & 5  & 88(1) & 5 & 426(460)\\%
\hline
SMSSync-464  & 4 & 984(88) & 4  & 1137(82) & 3& 1181(81) \\%sms
\hline
transistor-63    & 5  & 52(21) & 5 & 44(15) & 5 & 52(20)\\%transister
\hline
zom-271 & 5  & 277(283) & 5  & 202(74) & 5& 245(201)\\%zom
\hline
PixART-125  & 5  & 924(86)  & 5  & 1167(7) & 5 & 1719(253)\\%pixart-share
\hline
PixART-127  & 5 & 435(337) & 5 & 338(97) & 5  & 803(536) \\%pixart
\hline
ScreenCam-25  & 5 & 1545(943) & 5 & 1261(42) & 5  & 1265(37) \\%screencam
\hline
ventriloid-1& 4 & 150(103) & 4 & 108(83) & 0 & $>$(-)\\%ventriloid
\hline
Nextcloud-487  & 5& 310(461) & 5 & 509(556) & 5 & 1092(2) \\%Nextcloud
\hline
obdreader-22 & 5  & 1884(1717) & 5&  1862(1714) & 3 & 1216(142) \\%obdreader
\hline
dagger-46  & 5 & 25(3) & 5 & 24(1) & 5& 23(1) \\%dagger
\hline
ODK-2086  & 4 & 644(757) & 5 & 534(672) & 5 & 812(989)\\%ODK
\hline
k9-3255 & 4& 255(30) & 3  & 487(463) & 1 & 1022(-) \\%k9
\hline
k9-2612 & 5 & 152(20) & 5 & 102(17) & 5 & 1221(2550)\\%73
\hline
k9-2019 & 5 & 56(1) & 5 & 55(0) & 5 & 950(1214) \\%84
\hline
Anki-4586 & 5 & 205(277) & 5 & 275(324) & 1 & 987(-) \\
\hline
TagMo-12 & 5 & 14(0) & 5 & 17(5) & 5 & 14(0) \\
\hline
openMF-734  & 5 & 82(1) & 5 & 155(162) & 5 & 82(1)\\
\hline
FlashCards-13 & 5 & 140(11) & 5 & 135(9) & 5 & 137(10)\\
\hline
%\hline
%Total & 90\% & ?  & ?  & ? & ?  & ? & ?   & ? & ?  & ? & ?  & ?& ?\\
%\hline
\end{tabular}
%}
%\vspace*{-10pt}
\end{table}


\ignore{
\begin{table}[t!]
\vspace{1ex}
\centering
\scriptsize
\setlength{\tabcolsep}{1.5pt}
\caption{\label{tab:user}User Study for Manually Reproducing Crashes}
\scalebox{0.9}{
%\renewcommand{\arraystretch}{0.5}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
{\em Participant} & {\em U1} & {\em U2}
& {\em U3}& {\em U4}& {\em U5}& {\em U6}
& {\em U7}& {\em U8}& {\em U9}& {\em U10}
& {\em U11}& {\em U12}\\
\hline
App. (success) & 25/27 & 27/27& 25/27 & 22/27 & 24/27 &  25/27 & 24/27 & 22/27& 22/27 & 26/27& 26/27 & 25/27
\\
\hline
Time (total) & 7244  & 4758  & 8507 & 11136 & 9024 & 7576 & 9166 & 11672 & 12759 & 5677 & 5352 & 7744
\\
\hline
Useful (score) & 3 & 3 & 3 & 2 & 0 & 3 & 3 & 3 & 3 & 3 & 3 & 3
\\
\hline
\end{tabular}
}
%\normalsize
%\vspace*{-10pt}
\end{table}
}

\subsubsection{RQ4: Handling Low-Quality Bug Reports}

Columns 2--7 of Table~\ref{tab:user} reports the reproducibility of
\Name{} for the bug reports at the three different quality levels.  The
column \emph{success} indicates the number of mutated bug reports (out
of 5) that were successfully reproduced at each quality level.  The column
\emph{time} indicates the average time (and the standard deviation)
required for reproducing the crash.  The results show that among all
405 mutated bug reports for the three quality levels, \Name{} was able
to reproduce 93\%, 90\%, and 80\% of the bug crashes, respectively. Even when
50\% of the words were removed, \Name{} could still successfully reproduce 25
crashes,
%\commentty{where is 27 from}
better than the three baseline techniques.  
%The average times required
%for successfully reproducing the bug reports were 517, 637, and 814
%seconds for the three quality levels.  
The slowdowns caused by the
missing information with respect to the original bug reports were only
1.4x, 1.7x, and 2.2x, respectively.  These results suggest that
\emph{\Name{} can be used to handle low-quality bug reports with
  different levels of missing information.}

%\tingc{We may need to give more result analysis. Now we only show the results. }

\ignore{
\subsubsection{RQ5: Handling Bug Reports Generated by Different Users}

The last two columns of Table~\ref{tab:user} report the
reproducibility and cost (and standard deviation) of \Name{} for bug
reports re-written by the four participants. In total, \Name{}
successfully reproduced 102 out of 108 (94\%) bug reports, with an
average time of 552 seconds --- 32.6\% more time than reproducing the
original bug reports.  In six cases, \Name{} failed to reproduce the
crash due to the following reasons: 1) incorrect input values were
provided; 2) important steps were
missing; and 3) important words were misspelled.
%and 4) incorrect match between bug reports
%and the app GUI components. For the 4th reason, 
%a reporter wrote ``the app would be crashed and show a word".
%Since the word ``show"  is the same as the name of an app button,
%\Name{} incorrectly clicked this button and explored a number
%of irrelevant paths before reaching the timeout. 
%The average time required to reproduce the crashes is ??.
These results suggest that \emph{\Name{} is robust in handling
bug reports written by different users.}

}



==> study.tex <==
\section{Empirical Study}
\label{sec:study}

%We evaluated four major aspects of \Name{}, including
%1) the effectiveness and efficiency of \Name{} in reproducing
%crashing failures in bug reports, 2) the user experience of developers
%using \Name{}, and 3) the robustness of \Name{} in dealing
%with bug reports with different quality levels and written 
%by different users. To this end, we investigated four research questions: 


%To make our tool robust, 



To evaluate \Name{}, we consider four research questions:

\vspace*{3pt}
\noindent
{\bf RQ1:}
%
How effective and efficient is \Name{} at reproducing crashes
in bug reports?
%\tym{To what extent do the NLP techniques in 
%\Name{} affect its effectiveness and efficiency?
%}

\vspace*{3pt}
\noindent
{\bf RQ2:}
%
To what extent do the NLP techniques in 
\Name{} affect its effectiveness and efficiency?


\vspace*{3pt}
\noindent
{\bf RQ3:} 
%
Does \Name{} benefit developers compared to 
manual reproduction?

\vspace*{3pt}
\noindent
{\bf RQ4:} 
%
Can \Name{} reproduce crashes from 
different levels of low-quality bug reports?

\ignore{
\vspace*{3pt}
\noindent
{\bf RQ5:} 
%
How does 
%the effectiveness and efficiency of 
\Name{}  compare to 
%that of 
the other similar techniques?
}


\subsection{Datasets}

We selected bug reports and Android apps studied
by existing literature. To avoid overfitting,  we do not consider the 
the 813 Android bug reports that we used to identify the grammar
patterns.
%
Instead, we randomly crawled additional 330 bug reports 
containing the keywords ``crash"
and ``exception" from GitHub. 
%first included 162 bug reports from 68 apps 
%from an Android benchmark suite~\cite{choudhary2015automated}.
%
%\tingc{is this citation~\cite{azim2013targeted} correct? to my knowledge, that paper tests google play apps. Do we test google play apps?}.
%We then asked an undergraduate student who is not 
%familiar with our work to manually select 20 apps from GitHub. 
%We crawled the links of the issue tracking systems of these apps to
%obtain their bug reports. 
We next included all 15 bug reports from the
FUSION paper~\cite{moran2015auto} 
and 25 bug reports from a recent paper on translating Android bug reports 
into test cases~\cite{Fazzini2018}. 
FUSION considers the quality of these bug reports as low, so we wish to evaluate whether
\Name{} is capable of handling low-quality bug reports. 
%\tingc{can we mention more specific? e.g., how many total bug reports we have? how many can be successfully reproduced? what are the reasons why cannot reproduce?}
%\tym{We also included all bug reports from Yakusu~\cite{Fazzini2018}. }


We then manually filtered the 370 collected bug reports to get the final
set used in our experiments.  
This filtering was performed
independently by three graduate students, who have 2-4 years of
industrial software development experience.  
We first filtered bug reports involving actual app crashes, 
because \Name{} focuses on crash failures. This yielded 298 bug reports. 
We then filtered bug reports that 
could be reproduced manually by at least one inspector,
because some bugs could not be reproduced due to a lack of (or failed-to-compile) apks 
or environment issues.  
In total, we evaluated \Name{} on 51 bug
reports from 35 apks.  
%
\ignore{
The filtering process was
as follows: 1) reports involving app crashes (88), because \Name{} focuses
on crash failures; 2)
reports that could be reproduced manually by at least one inspector (?),
because some bugs could not be reproduced due to a lack of apks or
environment issues; 
3) reports that could be reproduced by Robotium
or UI Automator (?),
%since \Name{} depends on Robotium and UI Automator, 
because we wanted to isolate
bugs that were failing to reproduce due to the technical limitations of
the two execution engines  rather than
\Name{}.
%Following the above three steps yields us 15 apps  
%and 18 bug reports.  
%
%To amplify our datasets, we asked two other student inspectors, who
%are not familiar with our technique, to randomly select additional bug
%reports from GitHub issue trackers. This process followed the three
%criteria described above.  
In total, we evaluated \Name{} on 34 bug
reports from 27 apks.  
\commentty{need numbers}
%
%While larger number of bug reports may yield better evaluation,  
%the cost of the manual process is
%quite high -- preparation of the object  used in the study 
%required between 200 and 300 hours of researcher time.  
%Column Table~\ref{tab:objects} lists the details of the 20 bug reports. 
%\commentty{Make a table similar to Table 2 in FUSION paper.}
%
}
%
While larger number of bug reports may yield
better evaluation, the cost of the manual process is
quite high: preparation of the datasets
required between 300 and 400 hours of researcher time. 
%\tingc{We may need to give some evaluation setup info, e.g., the android sdk version we use, the configuration parameters of dynamic testing tools, the machine environment we run. All these information are important by considering we provide time measurement in Table II. In addition, we may need to mention a little about the implementation, i.e., the basic infrastructure we use.} 


\subsection{Implementation}

%To evaluate whether \Name{} can reproduce bug reports from real-world
%Android bugs, 

We conducted our experiment on
a physical X86 machine running with Ubuntu 14.04.  
The NLP techniques of \Name{} was implemented based on the spaCy 
dependency parser~\cite{spacy2}. 
The dynamic exploration component was implemented on 
top of two 
execution engines, Robotium~\cite{zadgaonkar2013robotium} and UI Automator~\cite{uiautomator},
for handling  apps compiled by a wide range
of Android SDK versions. 
An APK compiled by a lower version Android SDK ($<$ 6.0) 
can be handled by Robotium and that by a higher version SDK ($>$ 5.0)
can be handled by UI Automator.


\subsection{Experiment Design}
\label{sub:experiment}

\subsubsection{RQ1: Effectiveness and Efficiency of \Name{}}
%
We measure the effectiveness and efficiency of \Name{} in terms of whether it can successfully
reproduce crashes described in the bug reports within a time limit
(i.e., two hours) and efficiency in terms of the time it
took to reproduce each crash.



\subsubsection{RQ2: The Role of NLP in \Name{}}

Within \Name{}, we assess  whether the use of the NLP
techniques can affect
\Name{}'s effectiveness and efficiency.
We consider two ``vanilla" versions of \Name{}. 
The first version, \Name{}$_{N}$, is used to evaluate 
the effects of using grammar patterns. 
\Name{}$_{N}$ does not apply grammar patterns,
but only enables the second phase on dynamic matching. 
The second version is  \Name{}$_{D}$, which 
evaluates the effects of applying both grammar patterns 
and dynamic matching. 
The comparison between \Name{}$_{D}$ and \Name{}$_{N}$ can 
assess the effects of using dynamic matching. 
\Name{}$_{D}$  is a non-guided systematic GUI exploration technique. 
%

In fact,  \Name{}$_{D}$ is similar to existing Android 
bug detection tools~\cite{mao2016sapienz, monkey, su2017guided, azim2013targeted, amalfitano2012using},
which detect crashes in an unguided manner. 
\Name{}$_{D}$ was shown to be competitive with 
Monkey~\cite{monkey}, Sapienz~\cite{mao2016sapienz}, 
and the recent work Stoat~\cite{su2017guided} on our experiment subjects. 
The details can be found in our released artifacts~\cite{artifacts}.


\subsubsection{RQ3: Usefulness of \Name{}}
%
The goal of RQ3 is to evaluate the experience developer had using
\Name{} to reproduce bugs compared to using manual reproduction. We
recruited 12 graduate students as the participants.  All were familiar
with Android platforms and were experienced programmers. Each
participant read the 34 bug reports and tried to manually reproduce
the crashes. All apps were preinstalled.
%
For each bug report, the 12 participants timed how long it took for
them to understand the bug report and reproduce the bug.  If a
participant was not able to reproduce a bug after 30 minutes, that bug
was marked as not reproduced.  After the participants attempted to
reproduce all bugs, they were asked to use \Name{} on the
34 bug reports. This was followed by a survey
question: would you prefer to use \Name{} to reproduce bugs from bug
reports over manual reproduction?  Note that to avoid bias, the
participants were not aware of the purpose of this user study.
%To assess the results, we measure the
%time for reproducing the bugs, the number 
%of successful reproductions, and the responses to the survey questions.



\subsubsection{RQ4: Handling Low-Quality Bug Reports}
%
The goal of RQ4 is to assess the ability of \Name{} to handle
different levels of low-quality bug reports.  Since judging the
quality of a bug report is often subjective, we created low-quality
bug reports by randomly removing a set of words from 
the original bug reports.  
We focused on removing words from texts containing
reproducing steps. 
Specifically, we considered three variations for
each of the 27 bug report reports reproduced by \Name{} in order to
mimic different levels of quality: 1) removing 10\% of the words in
the report, 2) removing 20\% of the words in the report, and 3)
removing 50\% of the words in the report.  Due to the randomization of
removing words from bug reports, we repeated the removal operation
five times for each bug report across the three quality levels.  We
evaluate the effectiveness and efficiency of \Name{} in reproducing
crashes in the 405 ($27 \times 3 \times 5$) bug reports. 

%\tingc{pure randomly remove words. I remember one ASE reviewer mentions that removing words pure randomly is not convincing, %because some words may be more ``important'' than others. Should we give more details about how we remove words?}

\ignore{To
  assess the advantages of \Name{} in handling low-quality bug reports
  over manual reproduction, we then recruited five new participants to
  manually reproduce the mutated bug reports for the second quality
  level (i.e., removing 20\% of words).  }


\ignore{
\subsubsection{RQ5: Handling Bug Reports Generated by Different Users}

Given a bug, different reporters may describe it in different language
styles.  To assess the ability of \Name{} to handle bug reports
written by different users, we recruited another four participants to
write bug reports using a template similar to
Figure~\ref{fig:bugreport} for the 27 crashes reproduced by
\Name{}. To avoid introducing bias from the original bug reports, we
recorded videos of the steps needed to manually reproduce the crash
for every bug report. After viewing the video, each participant was
asked to write bug reports for the 27 crashes.  In total, the
participants constructed 108 bug reports. We then evaluated the
effectiveness and efficiency of \Name{} in reproducing the 108 bug
reports.
}

 

